Single Round-trip Hierarchical ORAM via Succinct Indices

Access patterns to data stored remotely create a side channel that is known to leak information even if the content of the data is encrypted. To protect against access pattern leakage, Oblivious RAM is a cryptographic primitive that obscures the (actual) access trace at the expense of additional access and periodic shuffling of the server's contents. A class of ORAM solutions, known as Hierarchical ORAM, has achieved theoretically \emph{optimal} logarithmic bandwidth overhead. However, to date, Hierarchical ORAMs are seen as only theoretical artifacts. This is because they require a large number of communication round-trips to locate (shuffled) elements at the server and involve complex building blocks such as cuckoo hash tables. To address the limitations of Hierarchical ORAM schemes in practice, we introduce Rank ORAM; the first Hierarchical ORAM that can retrieve data with a single round-trip of communication (as compared to a logarithmic number in previous work). To support non-interactive communication, we introduce a \emph{compressed} client-side data structure that stores, implicitly, the location of each element at the server. In addition, this location metadata enables a simple protocol design that dispenses with the need for complex cuckoo hash tables. Rank ORAM requires asymptotically smaller memory than existing (non-Hierarchical) state-of-the-art practical ORAM schemes (e.g., Ring ORAM) while maintaining comparable bandwidth performance. Our experiments on real network file-system traces demonstrate a reduction in client memory, against existing approaches, of a factor of~$100$. For example, when {outsourcing} a database of $17.5$TB, required client-memory is only $290$MB vs. $40$GB for standard approaches.

==> body/additional_proofs.tex <==
\section{Additional Proofs}

\subsection{Proof for Lemma \ref{lem:shortqueue}}
\label{app:lemma8}
We break down Lemma \ref{lem:shortqueue} into its components of fail rate, performance and security.
The algorithm fails if the temporary client storage exceeds $c\cdot \sqrt{n}$ for some constant $c$.
\begin{lemma}
On input array length $n$, \shortqueue fails with probability negligible in $n$.
\label{lem:fail_rate}
\end{lemma}
Before proving the result we require some probability tools.
\begin{definition}[Negative Association]
The random variables $X_1, \ldots, X_n$ are negatively associated if for all disjoint sets $ \mathbf{X}_1, \mathbf{X}_2 \subseteq \{X_1, \ldots, X_n\}$,
\begin{align*}
    \mathrm{E}[f(\mathbf{X}_1) \cdot g(\mathbf{X}_2)] \leq \mathrm{E}[f(\mathbf{X}_1)] \cdot \mathrm{E}[g(\mathbf{X}_2)],
\end{align*}
for all functions $f$ and $g$ that both non-increasing or both non-decreasing.
\end{definition}
This property, along with the following result, will be used to bound the size of the queues. 
\begin{lemma}[Lemma 2 of \cite{dubhashi1996balls}]
Let $X_1, \ldots, X_n$ be negatively associated random variables.
Then for non-decreasing functions $f_1, \ldots, f_k$ over disjoint sets $S_1, \ldots, S_k \subseteq \{ X_1, \ldots, X_n$\},
\begin{align*}
    \mathrm{E}\left[\prod_{i\in[k]} f_i(S_i) \right] &\leq \prod_{i\in[k]} \mathrm{E}\left[ f_i(S_i) \right]
\end{align*}
\label{lem:neg_ass_bounds}
\end{lemma}
Finally, we need the following result from Queuing Theory.
\begin{theorem}
Let $Q$ be a queue with batched arrival rate $1-\varepsilon$ and departure rate 1 and let $q_t$ be the size of the queue after $t$ batches of arrival. 
Then, for all $\varepsilon > 0, \mathrm{E}[e^{q_t}] \leq 2$.
\label{thm:queue_bound}
\end{theorem}


\begin{proof}[proof of Lemma \ref{lem:fail_rate}]
The goal is to bound the combined size of the queues during the execution of the algorithm.
To accomplish this, we construct a variant of \shortqueue that has the same functionality and fail rate.
We will prove that the fail rate for this variant is negligible.
The variant splits the input buckets $I_1, \ldots, I_{\sqrt{n}}$ in half and executes the first step of \shortqueue by reading the half-buckets in $2\sqrt{n}$ rounds.
After a half-bucket has been downloaded, \textit{one} item from each queue is uploaded to the temporary bucket at the server.
This is the only difference between the two.
As the ratio between the arrival and eviction rates at each queue is the same for both algorithms, they have identical fail rates. 
The variation allows us to use Theorem \ref{thm:queue_bound} with $\varepsilon = 0.5$.

Fixing notation, let $I^{\prime}_{2i}$ denote the first half of $I_{i}$, $I^{\prime}_{2{i+1}}$ denote the second half of $I_{i}$ and $X_{i,j}$ denote the number of addresses from $I^{\prime}_i$ that are placed in $Q_j$.
As the addresses from the input buckets are uniformly distributed across $Q_1,\ldots, Q_{\sqrt{n}}$, with $|I^{\prime}_i| = \sqrt{n}/2$, it holds that 
\begin{align}
    \mathrm{E}[X_{i,j}] = \frac{1}{2}.
    \label{eqn:arrival_rate}
\end{align}
Now, let $Y_{i,j}$ denote the length of $Q_j$ after $I^{\prime}_i$ has been read from the server.
Note that $Y_{i,j}$ is a non-decreasing function of the set of variables $\{X_{1,j}, \ldots, X_{i,j}\}$.
Let $Y_i = \sum_{j=1}^{\sqrt{n}} Y_{i,j}$.
To complete the proof, we need to bound ${Y_i}$ for all $2\sqrt{n}$ rounds.

The random variables $X_{i,1}, \ldots, X_{i,q}$ follow a balls-in-bins process.
Therefore, by Theorem 3.2 of \cite{dubhashi1996balls}, the variables are negatively associated.
Further, for all $i \neq j$, the sets $\{X_{i,1}, \ldots, X_{i,q}\}$ and $\{X_{j,1}, \ldots, X_{j,q}\}$ are mutually independent.
Therefore, the $Y_{i,j}$ are non-decreasing functions of disjoint sets of negatively associated random variables.
By Markov's Inequality,
\begin{align}
    \Pr[Y_i > c\cdot \sqrt{n}]
        &= \Pr[e^{\varepsilon Y_i}  > e^{\varepsilon c\cdot \sqrt{n}}] \nonumber\\
        &\leq e^{-\varepsilon c\cdot \sqrt{n}} \mathrm{E}\left[e^{\varepsilon Y_i}\right].
        \label{eqn:markov_bound}
\end{align}
By Equation \ref{eqn:arrival_rate}, the batched arrival rate is 0.5 and the departure rate is 1.
Therefore, by Theorem \ref{thm:queue_bound}, with $\varepsilon = 0.5$, 
\begin{align*}
    \mathrm{E}\left[e^{0.5 \cdot Y_i}\right] &= \mathrm{E}\left[\prod_{i=j}^{\sqrt{n}}e^{0.5 \cdot Y_{i,j}}\right] \\
    &\leq \prod_{j=1}^{\sqrt{n}} \mathrm{E}\left[ e^{0.5 \cdot Y_{i,j}} \right] \\ 
    &\leq 2^{\sqrt{n}}.
\end{align*}
The second inequality follows from Lemma \ref{lem:neg_ass_bounds}.
Thus, by inequality \ref{eqn:markov_bound}, with $\varepsilon=0.5$, 
\begin{align*}
    \Pr[Y_i > c\cdot \sqrt{n}] &\leq e^{-(c\cdot e/(1+e)-\ln 2)\sqrt{n}}.
\end{align*}
Therefore, by setting $c>(1+1/\varepsilon)\ln 2e$, $Y_i=\mathcal{O}(\sqrt{n})$ with probability at most $e^{-\mathcal{O}(1)\sqrt{n}}$.
Taking a union bound across all $2\sqrt{n}$ timesteps completes the result.
\end{proof}



We cover bandwidth and memory with the following result.
\begin{lemma}
On an input array of length $n$, the \shortqueue completes in $7n$ blocks of bandwidth and, on the condition that it does not fail, requires $\mathcal{O}(B \cdot \sqrt{n})$ bits of temporary private memory.
\end{lemma}
\begin{proof}
The memory claim comes from Lemma \ref{lem:fail_rate} and our definition of failure.
For the bandwidth, the first component of the algorithm downloads $n$ address and uploads $2n$ addresses.
The second component, in a sequence of rounds, downloads the full temporary array of length $2n$ and uploads it to the output array.
This leads to a total bandwidth cost of $7n$.
\end{proof}

\begin{lemma}
The \shortqueue is oblivious on functionality dummy shuffle (\textup{Definition} \ref{def:dummy_shuffle}).
\end{lemma}
\begin{proof}
We need to demonstrate that the access patterns produced by \shortqueue on two distinct inputs $\pi_1$ and $\pi_2$ are computationally indistinguishable to the adversary.
Let $\{I^{b}_i\}_{i \in \sqrt{n}}$ denote the input buckets for the execution of \shortqueue on $\pi_b$ for $b\in\{1,2\}$.
Both sets of input buckets are independent of their corresponding input permutations.
Similarly, let $X^{b}_{i,j}$ denote the number of addresses from $I^{b}_i$ that are placed in $Q^{b}_j$ for $b \in \{1,2\}$.
As the addresses are assigned uniformly at random to the sets $\{I^{b}_i\}_{i \in \sqrt{n}}$, $X^{1}_{i,j}$ is independent of $X^{2}_{i,j}$.
Therefore, for a fixed input array, the fail rate, which is observable to the adversary, is independent of the input permutation.

The set of buckets $\{I^{b}_i\}_{i \in \sqrt{n}}$ is independent of the input permutation.
Thus, the initial phase of downloading the input array appears as a sequence of uniformly random accesses.
The remaining accesses in the algorithm are identical for all inputs of the same length.
This completes the proof.
\end{proof}




==> body/histmem_proofs.tex <==

We break the proof up into a series of Lemmas focusing on [memory], update time and query times separately.
We begin the demonstration of the memory result.



\begin{restatable}{lemma}{histupdate}
On a database of size $n$, \historical supports updates in $\mathcal{O}(\log^2 n)$ amortized time.
\label{lem:histmem_update_app}
\end{restatable}

\begin{proof}
Following the schedule of \hierarchical, each update involves inserting an address into $\Phi_0$ and performing a merge.
For a merge into level $l$, in order to stay within our memory bounds, we extract the addresses from $\Phi_0 \cup \Phi_1 \cup \cdots \cup \Phi_{l-1}$, in sorted order, and build the run length code, on the fly, without resorting to a plain form representation.
To do this, we retrieve one address from the front of each code and place it in a list of length $l$.
Then, for $|\Phi_l|$ rounds we retrieve the smallest address from the list (deleting any duplicates) and place it in the next position of $\textsf{rle}(\Phi_l)$ by computing the corresponding run-length.
When an address is removed from the list, we retrieve the next address from the corresponding code by adding the next run-length to the removed address.

The list has length $l$ and we perform one scan per round.
Inserting a new run-length into $\Phi_l$ and extracting an address from a code both take constant time.
Therefore, a merge takes $\mathcal{O}(l \cdot |\Phi_l|)$ time.

The auxiliary structure can be built with one scan of the code.
For $W=\Theta(\log n)$, we read $W$ run-lengths at a time.
When we reach the start of each segment, we place the corresponding address and offset in the auxiliary structure.
This process completes in $|\Phi_l|$ time.

As a merge occurs every $|\Phi_l|$ updates, the amortized cost of merging into level $l$ is $\mathcal{O}(l)$.
Aggregated across all levels $\{0,1,\ldots,L-1\}$ (we do not perform a merge into level $\Phi_L$), this leads to an amortized update cost of 
\begin{align*}
    \sum_{l=0}^{L-1} \mathcal{O}(l) &= \mathcal{O}(L^2) = \mathcal{O}(\log^2 n).
\end{align*}
This completes the proof.

\end{proof}


\begin{restatable}{lemma}{histquery}
On a database of size $n$, \textup{\historical} admits \textup{\posll} and \textup{\level} queries in $\mathcal{O}(\log^2 n)$ time.
\label{lem:histmem_query_app}
\end{restatable}



\begin{proof}

We begin by evaluating the the cost of \rank, \index and \membership on the level dictionary $\Phi_l$.
The algorithmic details are available in Section \ref{subsec:auxiliary_ds}.
The code is divided into segments of width $\mathcal{O}(\log n)$.
The \rank and \membership operations involve two stages; (1) locate the correct segment in the code (as specified by the auxiliary structure); 
(2) scan the segment in search of the block address.
The auxiliary structure contains an ordered sequence of $\mathcal{O}(|\Phi_l|/ \log n)$ block addresses that correspond to the starting address of each segment.
Thus the forward pointer to the correct segment can be located, through a binary search, in $o(\log |\Phi_l|)$ time.
The subsequent linear scan can be executed in time proportional to the length of the segment.
Thus, both \rank and \membership require $\mathcal{O}(\log n)$ time to complete.
The \indll query does not require binary search on the auxiliary structure and can locate the correct segment in constant time. 
It also requires a linear scan of the segment and completes in $\mathcal{O}(\log n)$ time.

The $\level(x)$ function sequentially probes, from bottom to top, the dictionaries $\Phi = \{\Phi_0, \Phi_1, \ldots, \Phi_L\}$ with \membership queries.
In the worst-case, that is, when $x \in \Phi_L$, $L = \mathcal{O}(\log n)$ membership queries are preformed.
As each query takes $\mathcal{O}(\log n)$ time, the $\level$ function is evaluated in $\mathcal{O}(\log^2 n)$ time in the worst-case.
The $\posll(x)$ function requires one additional \rank query on $\Phi_{\level(x)}$ at a cost of $o(\log |\Phi_l|)$ time.
This completes the proof.
\end{proof}

\noindent Combined, Lemmas \ref{lem:histmem_update_app}-\ref{lem:histmem_query_app} serve as the proof for Lemma \ref{lem:query_times}.

==> body/outline-prev.tex <==
%\olya{some new text added here from the last subsection}
\rankoram is an ORAM solution that addresses concerns of adopting hierarchical ORAMs in practice.
It differs from prior instantiations of \hierarchical  by storing block metadata at the client. 
This results in two crucial improvements: first, we reduce the number of round-trips of communication per \access; and second, we can store blocks at the server in a simple and efficient data structure.
The latter improvement leads to a bandwidth and latency efficient \rebuild phase.

\olya{
At a high level, \rankoram follows the template of \hierarchical while keeping track of how recently each block has been accessed. A naive way of maintaining this information would require $\Theta(n \log n)$ bits. Instead we design a succinct data structure, called \historical, that requires only $O(n)$ bits and supports efficient update and lookup operations.} 

\olya{
In the rest of the section, we review the \hierarchical abstraction and then 
\if 0
allows the client to efficiently locate data blocks at the server and
There are two key building blocks that form the foundation of our protocol \rankoram.
The first is the \hierarchical abstraction that \rankoram implements.
\fi
present our client-side data structure \historical, which enables the performance improvements enjoyed by \rankoram.
%This section covers both of these building blocks.
At the end of the section, we show how to combine \hierarchical and \historical and present an overview of the \rankoram protocol.
}
%and illustrates how the two building blocks work together.

\subsection{\hierarchical}
\label{subsec:hierarchical}

The Hierarchical ORAM contains a hierarchy of oblivious hash tables $T_0, \ldots, T_L$, with $L = \log n$. In the words of Goldriech and Ostrovsky \cite{goldreich1996software}, the ORAM consists of ``a hierarchy of buffers of different sizes, where essentially we are going to access and shuffle buffers with frequency inversely proportional to their sizes''.
The \textit{hash table} abstraction contains a look-up query and a construction algorithm.
For the construction algorithm to be oblivious, by Definition~\ref{def:oblv_perm}, the input blocks must be placed in the table without leaking their locations through the access pattern.

A \hierarchical has the following structure.
The hash table~$T_l$ stores~$2^l$ data blocks.
Next to each table, a flag is stored to indicate whether the hash table is \textit{full} or \textit{empty}.
When receiving a request to an address,~$x$, the ORAM operation involves both an \access and \rebuild phase:
\begin{enumerate}
    \item \access: Access all non-empty hash tables in order and perform a lookup for address $x$. If the item is found in some level $l$, perform dummy look ups in the non-empty tables of $T_{l+1},\ldots, T_L$.
    If the operation is a $\readop$, then store the found data and place the block in $T_0$.
    If the operation is a $\writeop$, ignore the associated data and update the block with the fresh value.
    \item \rebuild: Find the smallest empty hash table $T_l$ (if no such level exists, then set $l=L$). 
    Merge the accessed item and all of $\{T_j\}_{j\leq l}$ into $T_l$.
    Mark levels $T_0, \ldots, T_{l-1}$ as empty.
\end{enumerate}
\noindent
A block is never accessed twice in the \textit{same}
hash table in between rebuilds at a given level.
This invariant is crucial to the security of the scheme.
As each block is always retrieved from a different location, the sequence of hash table probes produced by \hierarchical appears random to an adversary.

{Note that \access is interactive since the client does not know which level a block belongs to. 
That is, the client has to query the levels sequentially until the target block is found.}
This requires a round trip per level and increases  the latency of the protocol. 
{Our client-side data structure in \rankoram is designed to remove this cost}.
%A \rebuild can also be interactive.
%Therefore, we are also interested in the number of round-trips of communication required for each \rebuild operation.


\subsection{Client data structure}

\rankoram combines \hierarchical with a client-side data structure \historical.
Let $S_l = \{ v \mid (v,\square)\in T_l\}$
denote the set of logical addresses at level~$l$ in a \hierarchical. 
\historical maintains each set $S_l$, for $l\in [L-1]$, in a compressed indexed dictionary (as defined in Section \ref{sec:indexed}).
As access patterns typically have low entropy, for example, access patterns in file systems are highly sequential~\cite{oprea2007integrity},
the sets are compressible.


\historical, comprised of the collection of indexed dictionaries~$\mathcal{S}=\{S_1,\ldots, S_{L-1}\}$, \sloppy supports the following two functions:
\begin{align}
    \level(x) =  \min \{ i \mid (x,\square) \in T_i, i \in \{1, \ldots, L\}\}, \label{eqn:level}\\
    \posll(x) = 
    \begin{cases} 
        S_{\level(x)}.\rank(x) &\mbox{if } \textsf{level}(x) < L \\
        x & \mbox{if }\level(x) = L 
    \end{cases}.
    \label{eqn:position}
\end{align}
%An example of the \posll function is provided in Figure \ref{fig:acc}.
%\olya{could we please have an example here. we would like to hand hold the reader a bit that even if they do not follow the rest of the section they know exactly what this data structure stores and how it operates}
The function \level denotes the level a block belongs to
and is calculated in a sequence of membership queries starting from $S_0$ and progressing through the hierarchy.
The \level procedure is formalized in Algorithm \ref{alg:level}.
The function $\posll(x)$ denotes the \rank of address $x$ \textit{within} its current level. 
The \level functionality is observed in some prior work \cite{ren2014ring,stefanov2011towards}, where it is implemented in an array (called the position map) mapping element addresses to a collection of auxiliary information.
The \posll functionality is novel to this work and is used to map addresses into hash table locations.
An example of the \posll function for a given instance of \rankoram is given in Figure \ref{fig:acc}.

%\olya{Please add a similar examples to what you have for index and rank above and tie it to Figure 1, e.g.. }



When a \rebuild happens at the server ($T_{l}\gets \bigcup_{i=1}^{l-1} T_{i}$), \historical is updated accordingly:
\begin{align*}
    S_l &\gets \bigcup_{i=1}^{l-1} S_{l}\, \\
    \forall i \in \{1,\ldots, l-1\}: S_i &\gets \varnothing 
\end{align*}
Thus, one requirement for the choice of indexed dictionary is that it supports efficient merging.
Further, as each element belongs to exactly one level,
we do not need to store~$S_L$.
To evaluate Equation \eqref{eqn:level}, if the element is not a member of $\{S_l\}_{l \leq L-1}$, it must be a member of $S_L$.
Further, 
we do not need \rank information at level $L$.
This is covered in more detail in Subsection~\ref{sec:hash_table}.

The \level information is a function of block recency.
Consequently, \historical can be used to estimate the recency of a block.
This technique is similar to that used by Holland \textit{et al.} to estimate recency in small memory and with an arbitrary amount of relative error \cite{holland2020recency}.
Our work differs in the low-level details, such as the implementation of the component dictionaries, and with the additional requirement that we need to support \rank queries at each level.

To instantiate \historical, any indexed dictionary can be used.
For our result, we use run-length encoding \cite{bradley1969optimizing}.
The details are provided in Section \ref{SEC:CLIENT}.


\subsection{\rankoram overview}

%Our goal is to construct a \hierarchical that (1) incurs a constant number round-trips of communication per \access and \rebuild and (2) obtains a low concrete bandwidth overhead comparable to prior (non-hierarchical) state-of-the-art.
%At a high level, \rankoram follows the \hierarchical template outlined in Section \ref{subsec:hierarchical} and stores blocks at the server in a hierarchy of levels. 
\if 0
\rankoram differs from prior instantiations of \hierarchical by storing block metadata at the client. 
This results in two crucial improvements: first, we reduce the number of round-trips of communication per \access; and second, we can store blocks at the server in a simple and efficient data structure.
The latter improvement leads to a bandwidth and latency efficient \rebuild.
\fi

\rankoram builds on the observation that, in order to achieve a single round-trip, the client needs to know where a block is located, a priori, to avoid searching for it interactively at the server. 
To this end, \historical computes, for each block, its current level and its hash table position within the level. 
Subsequently, courtesy of this metadata, \historical informs the protocol of where to retrieve an accessed block and of where to retrieve dummies at the server.
Thus, all the level probes can be batched in a single non-interactive request to the server.

In addition, \historical allows us to improve the design of server-level storage and instantiate each level with an efficient permuted array, thus  dispensing with the (expensive) cuckoo hash table.
Hash tables are needed in \hierarchical to enable the efficient retrieval of elements in the domain $[1,n]$ from a table of size smaller than $n$ (that is, size $2^l$ at level~$l$). 
\historical compactly stores this mapping from the block domain to the hash table indices.
Therefore, a permuted array suffices as the level hash table. 
{Rebuilding a permuted array relies on a single call to an oblivious shuffle, making the \rebuild phase not only simpler than constructing a cuckoo hash table, but also more efficient (see Table~\ref{tab:hierarchical}).} 
%The mapping is computed from the \rank information encoded at each level.

\historical can be used by existing \hierarchical solutions that employ other hash tables to reduce round-trips of communication.
{However, we note that \historical cannot be used to encode metadata arrays for \ringoram and \partition, as these arrays do not exhibit temporal locality. 
For example, both constructions store arrays mapping addresses to random numbers.
These numbers not only contain high entropy, but are fixed for a given address between accesses.
In contrast, the level data stored in \historical is a function of block recency and changes with each \rebuild.


%We present an oblivious hash table solution that is enabled by the available client-side metadata and demonstrate how accesses are executed in a single round of communication.




==> body/server_comp.tex <==


To reduce the online bandwidth, we use a XOR trick, introduced by Dautrich \etal \cite{dautrich2014burst}, to reduce the size of the batch of requested blocks sent to the client by the server.
This optimization requires server-side computation.
The server's output from the \access request is a collection of encrypted dummies plus the encrypted target block.
Therefore, the server can XOR the ciphertexts together to produce a \textit{single} block to send to the client.
The client can unpack the retrieved element by assembling the corresponding collection of encrypted dummies and apply one XOR against the returned block. 
Formally, let $B_i$ denote the block the server retrieved from level $i$ and $l^{\prime}$ denote the level that contains the accessed block.
If the server returns the compressed batch $B_S = B_1 \oplus \cdots \oplus B_L$ (ingoring for simplicity the fact that some levels might be empty), 
the client can decode $B_{l^{\prime}}$ by first constructing 
\[
B_C = B_1 \oplus \cdots \oplus B_{l^{\prime}-1} \oplus B_{l^{\prime}+1} \oplus \cdots B_L
\]
as a collection of encrypted dummy blocks.
Then the client
performs
\[
B_{l^{\prime}} = B_S \oplus B_C.
\]
Note that this optimization requires server-side computation.
Nonetheless, this is a standard optimization from the literature \cite{dautrich2014burst,ren2014ring}.

This technique reduces online bandwidth from $1/2\log n$ to 1.
We summarize this result in the following Lemma.
\begin{lemma}
    With server-side computation, the online bandwidth cost for \rankoram is 1 and the amortized bandwidth cost is $3.5 \log n$.
\end{lemma}

==> body/shortqueueproof.tex <==

We break down Lemma \ref{LEM:SHORTQUEUE} into its components of fail rate, performance and security.
The algorithm fails if the temporary client storage exceeds $c\cdot \sqrt{n}$ for some constant $c$.
\begin{lemma}
On input array length $n$, \shortqueue fails with probability negligible in $n$.
\label{lem:fail_rate}
\end{lemma}
Before proving the result we require some probability tools.
\begin{definition}[Negative Association]
The random variables $X_1, \ldots, X_n$ are negatively associated if for all disjoint sets $ \mathbf{X}_1, \mathbf{X}_2 \subseteq \{X_1, \ldots, X_n\}$,
\begin{align*}
    \mathrm{E}[f(\mathbf{X}_1) \cdot g(\mathbf{X}_2)] \leq \mathrm{E}[f(\mathbf{X}_1)] \cdot \mathrm{E}[g(\mathbf{X}_2)],
\end{align*}
for all functions $f$ and $g$ that both non-increasing or both non-decreasing.
\end{definition}
This property, along with the following result, will be used to bound the size of the queues. 
\begin{lemma}[Lemma 2 of \cite{dubhashi1996balls}]
Let $X_1, \ldots, X_n$ be negatively associated random variables.
Then for non-decreasing functions $f_1, \ldots, f_k$ over disjoint sets $S_1, \ldots, S_k \subseteq \{ X_1, \ldots, X_n$\},
\begin{align*}
    \mathrm{E}\left[\prod_{i\in[k]} f_i(S_i) \right] &\leq \prod_{i\in[k]} \mathrm{E}\left[ f_i(S_i) \right]
\end{align*}
\label{lem:neg_ass_bounds}
\end{lemma}
Finally, we need the following result from Queuing Theory.
\begin{theorem}
Let $Q$ be a queue with batched arrival rate $1-\varepsilon$ and departure rate 1 and let $q_t$ be the size of the queue after $t$ batches of arrival. 
Then, for all $\varepsilon > 0, \mathrm{E}[e^{q_t}] \leq 2$.
\label{thm:queue_bound}
\end{theorem}


\begin{proof}[proof of Lemma \ref{lem:fail_rate}]
The goal is to bound the combined size of the queues during the execution of the algorithm.
To accomplish this, we construct a variant of \shortqueue that has the same functionality and fail rate.
We will prove that the fail rate for this variant is negligible.
The variant splits the input buckets $I_1, \ldots, I_{\sqrt{n}}$ in half and executes the first step of \shortqueue by reading the half-buckets in $2\sqrt{n}$ rounds.
After a half-bucket has been downloaded, \textit{one} item from each queue is uploaded to the temporary bucket at the server.
This is the only difference between the two.
As the ratio between the arrival and eviction rates at each queue is the same for both algorithms, they have identical fail rates. 
The variation allows us to use Theorem \ref{thm:queue_bound} with $\varepsilon = 0.5$.

Fixing notation, let $I^{\prime}_{2i}$ denote the first half of $I_{i}$, $I^{\prime}_{2{i+1}}$ denote the second half of $I_{i}$ and $X_{i,j}$ denote the number of addresses from $I^{\prime}_i$ that are placed in $Q_j$.
As the addresses from the input buckets are uniformly distributed across $Q_1,\ldots, Q_{\sqrt{n}}$, with $|I^{\prime}_i| = \sqrt{n}/2$, it holds that 
\begin{align}
    \mathrm{E}[X_{i,j}] = \frac{1}{2}.
    \label{eqn:arrival_rate}
\end{align}
Now, let $Y_{i,j}$ denote the length of $Q_j$ after $I^{\prime}_i$ has been read from the server.
Note that $Y_{i,j}$ is a non-decreasing function of the set of variables $\{X_{1,j}, \ldots, X_{i,j}\}$.
Let $Y_i = \sum_{j=1}^{\sqrt{n}} Y_{i,j}$.
To complete the proof, we need to bound ${Y_i}$ for all $2\sqrt{n}$ rounds.

The random variables $X_{i,1}, \ldots, X_{i,q}$ follow a balls-in-bins process.
Therefore, by Theorem 3.2 of \cite{dubhashi1996balls}, the variables are negatively associated.
Further, for all $i \neq j$, the sets $\{X_{i,1}, \ldots, X_{i,q}\}$ and $\{X_{j,1}, \ldots, X_{j,q}\}$ are mutually independent.
Therefore, the $Y_{i,j}$ are non-decreasing functions of disjoint sets of negatively associated random variables.
By Markov's Inequality,
\begin{align}
    \Pr[Y_i > c\cdot \sqrt{n}]
        &= \Pr[e^{\varepsilon Y_i}  > e^{\varepsilon c\cdot \sqrt{n}}] \nonumber\\
        &\leq e^{-\varepsilon c\cdot \sqrt{n}} \mathrm{E}\left[e^{\varepsilon Y_i}\right].
        \label{eqn:markov_bound}
\end{align}
By Equation \ref{eqn:arrival_rate}, the batched arrival rate is 0.5 and the departure rate is 1.
Therefore, by Theorem \ref{thm:queue_bound}, with $\varepsilon = 0.5$, 
\begin{align*}
    \mathrm{E}\left[e^{0.5 \cdot Y_i}\right] &= \mathrm{E}\left[\prod_{i=j}^{\sqrt{n}}e^{0.5 \cdot Y_{i,j}}\right] \\
    &\leq \prod_{j=1}^{\sqrt{n}} \mathrm{E}\left[ e^{0.5 \cdot Y_{i,j}} \right] \\ 
    &\leq 2^{\sqrt{n}}.
\end{align*}
The second inequality follows from Lemma \ref{lem:neg_ass_bounds}.
Thus, by inequality \ref{eqn:markov_bound}, with $\varepsilon=0.5$, 
\begin{align*}
    \Pr[Y_i > c\cdot \sqrt{n}] &\leq e^{-(c\cdot e/(1+e)-\ln 2)\sqrt{n}}.
\end{align*}
Therefore, by setting $c>(1+1/\varepsilon)\ln 2e$, $Y_i=\mathcal{O}(\sqrt{n})$ with probability at most $e^{-\mathcal{O}(1)\sqrt{n}}$.
Taking a union bound across all $2\sqrt{n}$ timesteps completes the result.
\end{proof}



We cover bandwidth and memory with the following result.
\begin{lemma}
On an input array of length $n$, the \shortqueue completes in $7n$ blocks of bandwidth and, on the condition that it does not fail, requires $\mathcal{O}(B \cdot \sqrt{n})$ bits of temporary private memory.
\end{lemma}
\begin{proof}
The memory claim comes from Lemma \ref{lem:fail_rate} and our definition of failure.
For the bandwidth, the first component of the algorithm downloads $n$ address and uploads $2n$ addresses.
The second component, in a sequence of rounds, downloads the full temporary array of length $2n$ and uploads it to the output array.
This leads to a total bandwidth cost of $7n$.
\end{proof}

\begin{lemma}
The \shortqueue is oblivious on functionality dummy shuffle (\textup{Definition} \ref{def:dummy_shuffle}).
\end{lemma}
\begin{proof}
We need to demonstrate that the access patterns produced by \shortqueue on two distinct inputs $\pi_1$ and $\pi_2$ are computationally indistinguishable to the adversary.
Let $\{I^{b}_i\}_{i \in \sqrt{n}}$ denote the input buckets for the execution of \shortqueue on $\pi_b$ for $b\in\{1,2\}$.
Both sets of input buckets are independent of their corresponding input permutations.
Similarly, let $X^{b}_{i,j}$ denote the number of addresses from $I^{b}_i$ that are placed in $Q^{b}_j$ for $b \in \{1,2\}$.
As the addresses are assigned uniformly at random to the sets $\{I^{b}_i\}_{i \in \sqrt{n}}$, $X^{1}_{i,j}$ is independent of $X^{2}_{i,j}$.
Therefore, for a fixed input array, the fail rate, which is observable to the adversary, is independent of the input permutation.

The set of buckets $\{I^{b}_i\}_{i \in \sqrt{n}}$ is independent of the input permutation.
Thus, the initial phase of downloading the input array appears as a sequence of uniformly random accesses.
The remaining accesses in the algorithm are identical for all inputs of the same length.
This completes the proof.
\end{proof}

